Interactive Code Generation via Test-Driven User-Intent Formalization

Large language models (LLMs) have shown great potential in automating significant aspects of coding by producing natural code from informal natural language (NL) intent. However, when interacting with LLMs, users have no guarantees that the code suggestions produced correctly satisfy the intent they provided. In fact, it is hard to define a notion of correctness since natural language can be ambiguous and lacks a formal semantics. In this paper, we propose the workflow of {\it interactive test-driven code generation}, which leverages lightweight user feedback to (a) formalize the user intent using generated tests that can be useful for debugging, and (b) produce an improved set of code suggestions by pruning and ranking candidate code suggestions. We describe a language-agnostic abstract algorithm and a concrete implementation TiCoder. We perform an automated evaluation of TiCoder on the \emph{MBPP} and \emph{HumanEval} code generation benchmarks. Our results are promising with using the OpenAI Codex LLM: our best algorithm improves the \passk{1} code generation accuracy (in absolute percentages) between $22.49\%$ to $37.71\%$ for MBPP and between $24.79\%$ to $53.98\%$ for HumanEval using between 1 to 5 simulated user queries.

==> ideal.tex <==
We begin by splitting the set $G$ of generated code suggestions into sets $G^+$ of correct suggestions (those that pass all the hidden tests in $T_p$) and $G^-$ of incorrect suggestions (those that fail an assertion in some test in $T_p$).
Then, we rank the tests from $U$ according to the following scoring metric $s_{\textit{ideal}}$ for each $t \in U$:

\begin{equation*}
    \begin{split}
        C_{(\textit{good,pass})} = & \left\{ c | c \in G^+ \land \textit{passes}(t, c) \right\} \\
        C_{(\textit{good,fail})} = & \left\{ c | c \in G^+ \land \lnot \textit{passes}(t, c) \right\} \\
        C_{(\textit{bad,pass})} = & \left\{ c | c \in G^- \land \textit{passes}(t, c) \right\} \\
        C_{(\textit{bad,fail})} = & \left\{ c | c \in G^- \land \lnot \textit{passes}(t, c) \right\} \\
        s_{\textit{ideal}}(t) = & \left\{
            \begin{array}{lr}
                (| C_{(\textit{bad,fail})} |, | C_{(\textit{good,pass})} |) & \text{if } \textit{passes}(t, \hat{c}) \\
                (| C_{(\textit{bad,pass})} |, | C_{(\textit{good,fail})} |) & \text{if } \textit{fails}(t, \hat{c}) \\
                (0, 0) & \text{otherwise}
            \end{array}
        \right\}
    \end{split}
\end{equation*}

Here, $\hat{c}$ is the ground truth reference solution.
The function $\textit{pass}(t, c)$ is true if a code $c$ passes the test $t$ without any errors.
Likewise, the function $\textit{fails}(t, c)$ is true if $c$ raises an \emph{assertion error} when run against $t$.
Note that it is possible for both $\textit{pass}(t, c)$ and $\textit{fails}(t, c)$ to be false in cases where $c$ crashes when run against $t$, but due to errors other than assertion errors, like syntax errors, precondition violations, and other issues.

Intuitively, the metric defines the score for a test $t$ based on the number of \emph{bad} code suggestions that can be pruned from $G$ if the user is presented with test $t$.
In cases where two tests prune the same number of bad code suggestions, we prioritize the one that will prune the smaller number of good code suggestions.
To determine the score, we simulate the user response for each test $t$ and consider 3 cases:
\aaditya{I think it might be better to use the \textit{SatisfiesUserIntent} function but I feel that its signature may be a bit different}
\begin{enumerate}
    \item If $t$ matches the user intent, i.e. if $\textit{pass}(t, \hat{c})$:
        In this case, we know that if the user is presented with test $t$, they would respond \textsc{Yes}, resulting in the code suggestions it does not pass being pruned from $G$.
        In such a case, we wish to prioritize a $t$ that the fewest bad codes and the most number of good codes pass on.
    \item If $t$ does not match the user intent, i.e. if $\textit{fails}(t, \hat{c})$:
        In this case, we know that if the user is presented with test $t$, they would respond \textsc{No}, resulting in the code suggestions it passes being pruned from $G$.
        In such a case, we wish to prioritize a $t$ that the most number of bad codes and the fewest good codes pass on.
    \item All other cases:
        Here, the user would respond \textsc{DontKnow} if presented with test $t$.
        Since we wish to minimize the chance of presenting such use cases to the user, we score these the lowest (0).
\end{enumerate}

This ranking is the ideal ranking since it considers the user intent while ranking each test suggestion, and definitively ranks suggestions that prune away the most number of bad codes the highest.
However, the requirement of knowing such a ground truth solution means that the ideal ranking policy is unrealizeable, and can only serve as an upper bound on any ranking policy.


==> tables/rq1.tex <==
\begin{table}
    \centering
    \begin{tabular}{l|c|c|c|c}
        Tool & pass@1@1 & pass@2@1 & pass@5@1 & pass@10@1 \\
        \hline
        Baseline & 48.61 (48.39) & 63.08 (62.89) & 75.58 (75.45) & 80.90 (80.83) \\
        Best & 70.49 (48.39) & 74.47 (60.89) & 79.39 (75.45) & 82.43 (80.83) \\
        IdealRanking & 85.65 & 87.90 & 88.88 & 89.22 \\
        IdealTests & 86.50 (48.39) & 88.61 (60.89) & 89.33 (75.45) & 89.45 (80.83) \\
    \end{tabular}
    \caption{Results of the accuracy experiment (pass@100 is 89.46\%) \shuvendu{why is pass@2@1 for Baseline 2percent higher?}}
    \label{tab:rq1}
\end{table}

==> tables/rq2.tex <==
\begin{table}
    \centering
    \begin{tabular}{l|c|c|c|c|c|c}
        Tool & pass@1@0 & pass@1@1 & pass@1@2 & pass@1@3 & pass@1@4 & pass@1@5 \\
        \hline
        Baseline & 48.39 & 48.61 & * & 50.14 & * & 50.98 \\
        \besttool{} & 48.39 & 70.49 & 76.11 & 78.92 & 83.14 & 85.48 \\
        IdealTests & 48.39 & 86.50 & 89.25 & 89.46 & 89.46 & 89.46 \\
    \end{tabular}
    \caption{Results of the user interaction experiment. \sakkas{replace IdealTests with ideal ranking hidden tests from onenote}. \sakkas{Best results for mq1 to mq5 in Best Option 1 (ranked codes) in onenote.}}
    \label{tab:rq2}
\end{table}

==> tables/rq4.tex <==
\begin{table}
    \centering
    \begin{tabular}{l||c|c|c|c||c}
         & \pass{1}{*} & \pass{2}{*} & \pass{5}{*} & \pass{10}{*} & Average number of queries \\
        \hline
        \emph{MBPP} & 76.23 & 80.39 & 84.07 & 86.52 & 1.7 \\
        \emph{HumanEval} & 58.39 & 67.08 & 75.78 & 81.99 & 1.5 \\
    \end{tabular}
    \caption{Results of the user interaction studies for stopping criteria (2). Here, the maximum possible number of user interactions is capped at 10.}
    \label{tab:rq4}
\end{table}
